Analysis on LLMs Performance for Code Summarization

Code summarization aims to generate concise natural language descriptions for source code. Deep learning has been used more and more recently in software engineering, particularly for tasks like code creation and summarization. Specifically, it appears that the most current Large Language Models with coding perform well on these tasks. Large Language Models (LLMs) have significantly advanced the field of code summarization, providing sophisticated methods for generating concise and accurate summaries of source code. This study aims to perform a comparative analysis of several open-source LLMs, namely LLaMA-3, Phi-3, Mistral, and Gemma. These models' performance is assessed using important metrics such as BLEU\textsubscript{3.1} and ROUGE\textsubscript{3.2}. Through this analysis, we seek to identify the strengths and weaknesses of each model, offering insights into their applicability and effectiveness in code summarization tasks. Our findings contribute to the ongoing development and refinement of LLMs, supporting their integration into tools that enhance software development and maintenance processes.

==> chapters/conclusion.tex <==
\chapter{Conclusion}\label{chapter:conclusion}

In conclusion, our evaluation of various large language models (LLMs) for code summarization reveals that Mistral-7b and Phi-3-medium are the top performers across multiple datasets. Mistral-7b consistently demonstrates superior capabilities, particularly excelling in JavaScript and PHP, while Phi-3-medium shows strong performance, especially in Ruby and Go. Llama-3-8b and Gemma-7b also produce decent results in specific datasets but generally fall behind the leading models. These findings highlight the importance of selecting the appropriate model based on the specific programming language and context. Future work should focus on further enhancing the understanding of code semantics and optimizing model efficiency to improve performance and applicability in real-world scenarios.

==> chapters/experiment.tex <==
\chapter{Experiment Setup}\label{chapter:experiment}

==> chapters/futureworks.tex <==
\chapter{Future Directions}\label{chapter:future}

The future direction for the comparative analysis of large language models (LLMs) in code summarization should encompass several key areas. First, expanding the evaluation to include a broader range of LLMs will provide a more comprehensive performance comparison, allowing for a better understanding of the strengths and weaknesses of different models. This can help in identifying the most suitable models for specific code summarization tasks. Second, enhancing the model's understanding of code semantics, beyond mere syntax, is crucial. Improving the semantic comprehension will lead to higher quality summaries that accurately capture the intent and functionality of the code, rather than just its structure. Lastly, focusing on reducing latency and computational requirements is essential to make the models more efficient and practical for real-world applications. This can be achieved through optimization techniques and more efficient model architectures, ensuring that the benefits of advanced LLMs are accessible without prohibitive computational costs.  

==> chapters/limitation.tex <==
\chapter{Discussion}\label{chapter:discussion}

\subsection{Limitation}
Each model may require individualized training strategies to accommodate differences in architecture and learning dynamics, despite being subjected to the same initial conditions. The availability and quality of training data are critical yet challenging, as high-quality, domain-specific datasets for code summarization are scarce. This scarcity can hinder the models' ability to generalize effectively to diverse real-world coding practices. Additionally, ensuring that each model's output is not only accurate but also contextually relevant to developers is a complex task that involves balancing technical accuracy with practical usability. These challenges highlight the need for a nuanced approach to training and evaluating each model within your research framework.

Another critical limitation is the potential for model bias. Since LLMs are trained on available data, any inherent biases in this data can be amplified during training and fine-tuning. This could lead to models that perform well on certain types of code or coding styles but poorly on others, potentially affecting the fairness and inclusivity of the tool.

Code practices and programming languages evolve, so models trained on current datasets may quickly become outdated. Continuously updating the models to adapt to new programming paradigms or languages is a significant challenge, requiring ongoing collection of new data and retraining.



\subsection{Future Direction}

The future direction for the comparative analysis of large language models (LLMs) in code summarization should encompass several key areas. First, expanding the evaluation to include a broader range of LLMs will provide a more comprehensive performance comparison, allowing for a better understanding of the strengths and weaknesses of different models. This can help in identifying the most suitable models for specific code summarization tasks. Second, enhancing the model's understanding of code semantics, beyond mere syntax, is crucial. Improving the semantic comprehension will lead to higher quality summaries that accurately capture the intent and functionality of the code, rather than just its structure. Lastly, focusing on reducing latency and computational requirements is essential to make the models more efficient and practical for real-world applications. This can be achieved through optimization techniques and more efficient model architectures, ensuring that the benefits of advanced LLMs are accessible without prohibitive computational costs.  


\subsection{Conclusion}

In conclusion, our evaluation of various large language models (LLMs) for code summarization reveals that Mistral-7b and Phi-3-medium are the top performers across multiple datasets. Mistral-7b consistently demonstrates superior capabilities, particularly excelling in JavaScript and PHP, while Phi-3-medium shows strong performance, especially in Ruby and Go. Llama-3-8b and Gemma-7b also produce decent results in specific datasets but generally fall behind the leading models. These findings highlight the importance of selecting the appropriate model based on the specific programming language and context. Future work should focus on further enhancing the understanding of code semantics and optimizing model efficiency to improve performance and applicability in real-world scenarios.
